Class-Incremental Learning for Action Recognition in Videos

We tackle catastrophic forgetting problem in the context of class-incremental learning for video recognition, which has not been explored actively despite the popularity of continual learning. Our framework addresses this challenging task by introducing time-channel importance maps and exploiting the importance maps for learning the representations of incoming examples via knowledge distillation. We also incorporate a regularization scheme in our objective function, which encourages individual features obtained from different time steps in a video to be uncorrelated and eventually improves accuracy by alleviating catastrophic forgetting. We evaluate the proposed approach on brand-new splits of class-incremental action recognition benchmarks constructed upon the UCF101, HMDB51, and Something-Something V2 datasets, and demonstrate the effectiveness of our algorithm in comparison to the existing continual learning methods that are originally designed for image data.

==> figure/ucf_10.tex <==
%!TEX root = ../06577.tex

\pgfplotsset{
every axis plot/.append style={line width=0.8pt},
tick label style={font=\scriptsize},
%label style={font=\small},
label style={font=\footnotesize},
legend style={font=\scriptsize, at={(0.01,0.01)},anchor=south west}
%legend style={font=\scriptsize, at={(1,1)},anchor=north east}
}

\pgfplotsset{compat=1.12}

\begin{tikzpicture}
    \begin{axis}[
      height=6.0cm, %\textwidth,%7.5cm,
      width=6.0cm,
      xlabel = Number of classes,
      ylabel = Accuracy over seen classes,
      x label style={scale=0.9,at={(axis description cs:0.5,-0.07)},anchor=north},
      %y label style={at={(axis description cs:-0.1,.5)},rotate=90,anchor=south},
      y label style={scale=0.9,at={(axis description cs:-0.1,0.5)},anchor=south},
      xtick={51,61,71,81,91,101},
      xmin = 48,
      xmax = 105,
      ymin = 55.0,
      ymax = 90.0,
      legend style={nodes={scale=0.7,inner sep=1pt,text depth=0.0em}}]
    ]
    \input{figure/data/ucf_10/ours_nme}
    \input{figure/data/ucf_10/ours_cnn}
    \input{figure/data/ucf_10/pod_nme}
    \input{figure/data/ucf_10/pod_cnn}
    \input{figure/data/ucf_10/ucir_nme}
    \input{figure/data/ucf_10/ucir_cnn}
    %\input{figure/data/memory_5}
    %\input{figure/data/memory_2}
    %\input{figure/data/memory_1}   
  

    \legend{
       Ours (NME) (77.16) \\
       Ours (CNN) (74.89) \\
       PODNet (NME) (74.37) \\
       PODNet (CNN) (73.26) \\
       UCIR (NME) (74.09) \\
       UCIR (CNN) (74.31) \\
    }
    \end{axis}
\end{tikzpicture}
